Imagen Video: High Definition Video Generation with Diffusion Models

We present Imagen Video, a text-conditional video generation system based on a cascade of video diffusion models. Given a text prompt, Imagen Video generates high definition videos using a base video generation model and a sequence of interleaved spatial and temporal video super-resolution models. We describe how we scale up the system as a high definition text-to-video model including design decisions such as the choice of fully-convolutional temporal and spatial super-resolution models at certain resolutions, and the choice of the v-parameterization of diffusion models. In addition, we confirm and transfer findings from previous work on diffusion-based image generation to the video generation setting. Finally, we apply progressive distillation to our video models with classifier-free guidance for fast, high quality sampling. We find Imagen Video not only capable of generating videos of high fidelity, but also having a high degree of controllability and world knowledge, including the ability to generate diverse videos and text animations in various artistic styles and with 3D object understanding. See https://imagen.research.google/video/ for samples.

==> distilled_samples_figure.tex <==
\begin{figure}
\centering
\setlength{\tabcolsep}{2pt}
    \begin{tabular}{ccccc}
         \includegraphics[width=0.2\textwidth]{frames/Wooden figurine surfing on a surfboard in space./frame_0.jpeg} &
         \includegraphics[width=0.2\textwidth]{frames/Wooden figurine surfing on a surfboard in space./frame_28.jpeg} &
         \includegraphics[width=0.2\textwidth]{frames/Wooden figurine surfing on a surfboard in space./frame_56.jpeg} &
         \includegraphics[width=0.2\textwidth]{frames/Wooden figurine surfing on a surfboard in space./frame_85.jpeg} &
         \includegraphics[width=0.2\textwidth]{frames/Wooden figurine surfing on a surfboard in space./frame_113.jpeg} \\
         \includegraphics[width=0.2\textwidth]{frames/Balloon full of water exploding in extreme slow motion./frame_0.jpeg} &
         \includegraphics[width=0.2\textwidth]{frames/Balloon full of water exploding in extreme slow motion./frame_14.jpeg} &
         \includegraphics[width=0.2\textwidth]{frames/Balloon full of water exploding in extreme slow motion./frame_28.jpeg} &
         \includegraphics[width=0.2\textwidth]{frames/Balloon full of water exploding in extreme slow motion./frame_85.jpeg} &
         \includegraphics[width=0.2\textwidth]{frames/Balloon full of water exploding in extreme slow motion./frame_113.jpeg} \\
    \end{tabular}
    \caption{Snapshots of frames from videos generated by Imagen Video for the text prompts \textit{Wooden figurine surfing on a surfboard in space} (top row), and \textit{Balloon full of water exploding in extreme slow motion} (bottom row).}
    \label{fig:video_frames_figure}
\end{figure}


==> interesting_properties.tex <==
\begin{figure}
\centering
\setlength{\tabcolsep}{2pt}
    \begin{tabular}{ccccc}
         \includegraphics[width=0.2\textwidth]{frames/3d_sushi_car/imagenvideo_0.png} &
         \includegraphics[width=0.2\textwidth]{frames/3d_sushi_car/imagenvideo_36.png} &
         \includegraphics[width=0.2\textwidth]{frames/3d_sushi_car/imagenvideo_73.png} &
         \includegraphics[width=0.2\textwidth]{frames/3d_sushi_car/imagenvideo_109.png} &
         \includegraphics[width=0.2\textwidth]{frames/3d_sushi_car/imagenvideo_128.png} \\
        \multicolumn{5}{c}{\footnotesize A 3D model of a car made out of sushi. Studio lighting.} \\
          
         \includegraphics[width=0.2\textwidth]{frames/image_sprouts_fairytale/imagenvideo_0.jpeg} &
         \includegraphics[width=0.2\textwidth]{frames/image_sprouts_fairytale/imagenvideo_18.jpeg} &
         \includegraphics[width=0.2\textwidth]{frames/image_sprouts_fairytale/imagenvideo_36.jpeg} &
         \includegraphics[width=0.2\textwidth]{frames/image_sprouts_fairytale/imagenvideo_54.jpeg} &
         \includegraphics[width=0.2\textwidth]{frames/image_sprouts_fairytale/imagenvideo_128.jpeg} \\
         \multicolumn{5}{c}{\footnotesize Sprouts in the shape of text 'Imagen' coming out of a fairytale book.} \\
         
       
         
        \includegraphics[width=0.2\textwidth]{frames/cat_eating_gogh/0000.jpeg} &
        \includegraphics[width=0.2\textwidth]{frames/cat_eating_gogh/0032.jpeg} &
        \includegraphics[width=0.2\textwidth]{frames/cat_eating_gogh/0064.jpeg} &
        \includegraphics[width=0.2\textwidth]{frames/cat_eating_gogh/0096.jpeg} &
        \includegraphics[width=0.2\textwidth]{frames/cat_eating_gogh/0128.jpeg} \\
        \multicolumn{5}{c}{\footnotesize A cat eating food out of a bowl, in style of van Gogh.} \\[10pt]
    \end{tabular}
    \caption{Snapshots of frames from videos generated by Imagen Video demonstrating interesting properties of the model. \textit{(Top)} The model is able to implicitly understand the 3D structure of objects. \textit{(Middle)} The model is able to render accurate text with realistic dynamics. \textit{(Bottom)} The joint training with images and videos allows the model to generate dynamics these interesting settings.}
    \label{fig:interesting_properties}
\end{figure}

